Eigenvalue estimates for the poly-Laplace operator on lattice subgraphs

We introduce the discrete poly-Laplace operator on a subgraph with Dirichlet boundary condition. We obtain upper and lower bounds for the sum of the first $k$ Dirichlet eigenvalues of the poly-Laplace operators on a finite subgraph of lattice graph $\mathbb{Z}^{d}$ extending classical results of Li-Yau and Kr\"oger. Moreover, we prove that the Dirichlet $2l$-order poly-Laplace eigenvalues are at least as large as the squares of the Dirichlet $l$-order poly-Laplace eigenvalues.

==> poly-laplace_ref.tex <==
@article {Weyl1912,
    AUTHOR = {Weyl, Hermann},
     TITLE = {Das asymptotische {V}erteilungsgesetz der {E}igenwerte
              linearer partieller {D}ifferentialgleichungen (mit einer
              {A}nwendung auf die {T}heorie der {H}ohlraumstrahlung)},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {71},
      YEAR = {1912},
    NUMBER = {4},
     PAGES = {441--479},
      ISSN = {0025-5831,1432-1807},
   MRCLASS = {99-04},
  MRNUMBER = {1511670},
       DOI = {10.1007/BF01456804},
       URL = {https://doi.org/10.1007/BF01456804},
}

@article {Polya1961,
    AUTHOR = {P\'olya, G.},
     TITLE = {On the eigenvalues of vibrating membranes},
   JOURNAL = {Proc. London Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {11},
      YEAR = {1961},
     PAGES = {419--433},
      ISSN = {0024-6115,1460-244X},
   MRCLASS = {73.35 (35.80)},
  MRNUMBER = {129219},
MRREVIEWER = {H.\ F.\ Weinberger},
       DOI = {10.1112/plms/s3-11.1.419},
       URL = {https://doi.org/10.1112/plms/s3-11.1.419},
}

@incollection {Lieb1980,
    AUTHOR = {Lieb, Elliott H.},
     TITLE = {The number of bound states of one-body {S}chroedinger
              operators and the {W}eyl problem},
 BOOKTITLE = {Geometry of the {L}aplace operator ({P}roc. {S}ympos. {P}ure
              {M}ath., {U}niv. {H}awaii, {H}onolulu, {H}awaii, 1979)},
    SERIES = {Proc. Sympos. Pure Math.},
    VOLUME = {XXXVI},
     PAGES = {241--252},
 PUBLISHER = {Amer. Math. Soc., Providence, RI},
      YEAR = {1980},
      ISBN = {0-8218-1439-7},
   MRCLASS = {35P05 (81F05)},
  MRNUMBER = {573436},
MRREVIEWER = {Christian\ Gruber},
}

@article {Li1983,
    AUTHOR = {Li, Peter and Yau, Shing Tung},
     TITLE = {On the {S}chr\"odinger equation and the eigenvalue problem},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {88},
      YEAR = {1983},
    NUMBER = {3},
     PAGES = {309--318},
      ISSN = {0010-3616,1432-0916},
   MRCLASS = {58G25 (35P99 58G05 81C05)},
  MRNUMBER = {701919},
MRREVIEWER = {Harold\ Donnelly},
       URL = {http://projecteuclid.org/euclid.cmp/1103922378},
}

@article {Berezin1972,
    AUTHOR = {Berezin, F. A.},
     TITLE = {Covariant and contravariant symbols of operators},
   JOURNAL = {Izv. Akad. Nauk SSSR Ser. Mat.},
  FJOURNAL = {Izvestiya Akademii Nauk SSSR. Seriya Matematicheskaya},
    VOLUME = {36},
      YEAR = {1972},
     PAGES = {1134--1167},
      ISSN = {0373-2436},
   MRCLASS = {47B99 (81.47)},
  MRNUMBER = {350504},
MRREVIEWER = {W.\ Faris},
}

@article {Melas2003,
    AUTHOR = {Melas, Antonios D.},
     TITLE = {A lower bound for sums of eigenvalues of the {L}aplacian},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {131},
      YEAR = {2003},
    NUMBER = {2},
     PAGES = {631--636},
      ISSN = {0002-9939,1088-6826},
   MRCLASS = {35P20 (35J25 58J50)},
  MRNUMBER = {1933356},
MRREVIEWER = {Lech\ Zielinski},
       DOI = {10.1090/S0002-9939-02-06834-X},
       URL = {https://doi.org/10.1090/S0002-9939-02-06834-X},
}

@article {Kovarik2009,
    AUTHOR = {Kova\v r\'ik, Hynek and Vugalter, Semjon and Weidl, Timo},
     TITLE = {Two-dimensional {B}erezin-{L}i-{Y}au inequalities with a
              correction term},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {287},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {959--981},
      ISSN = {0010-3616,1432-0916},
   MRCLASS = {58J50 (35J05 35P15)},
  MRNUMBER = {2486669},
MRREVIEWER = {G\"unter\ Berger},
       DOI = {10.1007/s00220-008-0692-1},
       URL = {https://doi.org/10.1007/s00220-008-0692-1},
}

@article {Yolcu2012,
    AUTHOR = {Yolcu, Selma Y\i ld\i r\i m{} and Yolcu, T\"urkay},
     TITLE = {Multidimensional lower bounds for the eigenvalues of {S}tokes
              and {D}irichlet {L}aplacian operators},
   JOURNAL = {J. Math. Phys.},
  FJOURNAL = {Journal of Mathematical Physics},
    VOLUME = {53},
      YEAR = {2012},
    NUMBER = {4},
     PAGES = {043508, 17},
      ISSN = {0022-2488,1089-7658},
   MRCLASS = {35Q35 (35P15)},
  MRNUMBER = {2953152},
       DOI = {10.1063/1.3701978},
       URL = {https://doi.org/10.1063/1.3701978},
}

@article {Kroger1994,
    AUTHOR = {Kr\"oger, Pawel},
     TITLE = {Estimates for sums of eigenvalues of the {L}aplacian},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {126},
      YEAR = {1994},
    NUMBER = {1},
     PAGES = {217--227},
      ISSN = {0022-1236,1096-0783},
   MRCLASS = {58G25 (35P15 58G20)},
  MRNUMBER = {1305068},
MRREVIEWER = {Sylvie\ Desjardins},
       DOI = {10.1006/jfan.1994.1146},
       URL = {https://doi.org/10.1006/jfan.1994.1146},
}

@article {Kroger1992,
    AUTHOR = {Kr\"oger, P.},
     TITLE = {Upper bounds for the {N}eumann eigenvalues on a bounded domain
              in {E}uclidean space},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {106},
      YEAR = {1992},
    NUMBER = {2},
     PAGES = {353--357},
      ISSN = {0022-1236,1096-0783},
   MRCLASS = {47F05 (35J05 35P15)},
  MRNUMBER = {1165859},
       DOI = {10.1016/0022-1236(92)90052-K},
       URL = {https://doi.org/10.1016/0022-1236(92)90052-K},
}

@article {Strichartz1996,
    AUTHOR = {Strichartz, Robert S.},
     TITLE = {Estimates for sums of eigenvalues for domains in homogeneous
              spaces},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {137},
      YEAR = {1996},
    NUMBER = {1},
     PAGES = {152--190},
      ISSN = {0022-1236,1096-0783},
   MRCLASS = {58G25 (35P20)},
  MRNUMBER = {1383015},
MRREVIEWER = {Jacques\ Faraut},
       DOI = {10.1006/jfan.1996.0043},
       URL = {https://doi.org/10.1006/jfan.1996.0043},
}

@book {Henrot2006,
    AUTHOR = {Henrot, Antoine},
     TITLE = {Extremum problems for eigenvalues of elliptic operators},
    SERIES = {Frontiers in Mathematics},
 PUBLISHER = {Birkh\"auser Verlag, Basel},
      YEAR = {2006},
     PAGES = {x+202},
      ISBN = {978-3-7643-7705-2; 3-7643-7705-4},
   MRCLASS = {35P05 (35J05 35J15 35P15 47F05 49R50)},
  MRNUMBER = {2251558},
MRREVIEWER = {G\"unter\ Berger},
}

@article {Agmon1965,
    AUTHOR = {Agmon, Shmuel},
     TITLE = {On kernels, eigenvalues, and eigenfunctions of operators
              related to elliptic problems},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {18},
      YEAR = {1965},
     PAGES = {627--663},
      ISSN = {0010-3640,1097-0312},
   MRCLASS = {47.65 (35.80)},
  MRNUMBER = {198287},
MRREVIEWER = {A.\ Friedman},
       DOI = {10.1002/cpa.3160180405},
       URL = {https://doi.org/10.1002/cpa.3160180405},
}

@article {Pleijel1950,
    AUTHOR = {Pleijel, \AA ke},
     TITLE = {On the eigenvalues and eigenfunctions of elastic plates},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {3},
      YEAR = {1950},
     PAGES = {1--10},
      ISSN = {0010-3640,1097-0312},
   MRCLASS = {36.0X},
  MRNUMBER = {37459},
MRREVIEWER = {J.\ B.\ Diaz},
       DOI = {10.1002/cpa.3160030102},
       URL = {https://doi.org/10.1002/cpa.3160030102},
}

@book {Birman1980,
    AUTHOR = {Birman, M. \v S. and Solomjak, M. Z.},
     TITLE = {Quantitative analysis in {S}obolev imbedding theorems and
              applications to spectral theory},
    SERIES = {American Mathematical Society Translations, Series 2},
    VOLUME = {114},
      NOTE = {Translated from the Russian by F. A. Cezus},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {1980},
     PAGES = {viii+132},
      ISBN = {0-8218-3064-3},
   MRCLASS = {46E35 (35P20)},
  MRNUMBER = {562305},
}

@article{Birman1979,
  title={Asymptotic behavior of the spectrum of differential equations},
  author={Birman, M Sh and Solomyak, MZ},
  journal={Journal of Soviet Mathematics},
  volume={12},
  pages={247--283},
  year={1979},
  publisher={Springer}
}

@article {Levine1985,
    AUTHOR = {Levine, H. A. and Protter, M. H.},
     TITLE = {Unrestricted lower bounds for eigenvalues for classes of
              elliptic equations and systems of equations with applications
              to problems in elasticity},
   JOURNAL = {Math. Methods Appl. Sci.},
  FJOURNAL = {Mathematical Methods in the Applied Sciences},
    VOLUME = {7},
      YEAR = {1985},
    NUMBER = {2},
     PAGES = {210--222},
      ISSN = {0170-4214,1099-1476},
   MRCLASS = {35P15 (35J99 73C02)},
  MRNUMBER = {797333},
MRREVIEWER = {L.\ E.\ Payne},
       DOI = {10.1002/mma.1670070113},
       URL = {https://doi.org/10.1002/mma.1670070113},
}

@article {Chen2013,
    AUTHOR = {Cheng, Qing-Ming and Qi, Xuerong and Wei, Guoxin},
     TITLE = {A lower bound for eigenvalues of the poly-{L}aplacian with
              arbitrary order},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {262},
      YEAR = {2013},
    NUMBER = {1},
     PAGES = {35--47},
      ISSN = {0030-8730,1945-5844},
   MRCLASS = {35P15 (35J40 35P20)},
  MRNUMBER = {3069054},
MRREVIEWER = {Francesco\ Della Pietra},
       DOI = {10.2140/pjm.2013.262.35},
       URL = {https://doi.org/10.2140/pjm.2013.262.35},
}

@article {Wei2016,
    AUTHOR = {Wei, Guoxin and Zeng, Lingzhong},
     TITLE = {Estimates for eigenvalues of poly-harmonic operators},
   JOURNAL = {Adv. Nonlinear Stud.},
  FJOURNAL = {Advanced Nonlinear Studies},
    VOLUME = {16},
      YEAR = {2016},
    NUMBER = {1},
     PAGES = {31--44},
      ISSN = {1536-1365,2169-0375},
   MRCLASS = {35J40 (35P15)},
  MRNUMBER = {3456744},
       DOI = {10.1515/ans-2015-5020},
       URL = {https://doi.org/10.1515/ans-2015-5020},
}

@article {Yildirim2014,
    AUTHOR = {Y\i ld\i r\i m{} Yolcu, Selma and Yolcu, T\"urkay},
     TITLE = {Eigenvalue bounds for the poly-harmonic operators},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {58},
      YEAR = {2014},
    NUMBER = {3},
     PAGES = {847--865},
      ISSN = {0019-2082,1945-6581},
   MRCLASS = {35P15 (35J40 35P20)},
  MRNUMBER = {3395965},
MRREVIEWER = {Osanobu\ Yamada},
       URL = {http://projecteuclid.org/euclid.ijm/1441790392},
}

@article {Cheng2013,
    AUTHOR = {Cheng, Qing-Ming and Wei, Guoxin},
     TITLE = {Upper and lower bounds for eigenvalues of the clamped plate
              problem},
   JOURNAL = {J. Differential Equations},
  FJOURNAL = {Journal of Differential Equations},
    VOLUME = {255},
      YEAR = {2013},
    NUMBER = {2},
     PAGES = {220--233},
      ISSN = {0022-0396,1090-2732},
   MRCLASS = {35J40 (35P15)},
  MRNUMBER = {3047401},
MRREVIEWER = {Salvador\ Villegas},
       DOI = {10.1016/j.jde.2013.04.004},
       URL = {https://doi.org/10.1016/j.jde.2013.04.004},
}




@article {Jost2011,
    AUTHOR = {Jost, J\"urgen and Li-Jost, Xianqing and Wang, Qiaoling and
              Xia, Changyu},
     TITLE = {Universal bounds for eigenvalues of the polyharmonic
              operators},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {363},
      YEAR = {2011},
    NUMBER = {4},
     PAGES = {1821--1854},
      ISSN = {0002-9947,1088-6850},
   MRCLASS = {35P15 (31B30 35J40 35P20 35R01)},
  MRNUMBER = {2746667},
MRREVIEWER = {Konstantin\ Yu.\ Fedorovski\u i},
       DOI = {10.1090/S0002-9947-2010-05147-5},
       URL = {https://doi.org/10.1090/S0002-9947-2010-05147-5},
}

@article {Forster2008,
    AUTHOR = {F\"orster, Clemens and \"Ostensson, J\"orgen},
     TITLE = {Lieb-{T}hirring inequalities for higher order differential
              operators},
   JOURNAL = {Math. Nachr.},
  FJOURNAL = {Mathematische Nachrichten},
    VOLUME = {281},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {199--213},
      ISSN = {0025-584X,1522-2616},
   MRCLASS = {35P15 (35J30 47F05)},
  MRNUMBER = {2387360},
MRREVIEWER = {M.\ S.\ Agranovich},
       DOI = {10.1002/mana.200510595},
       URL = {https://doi.org/10.1002/mana.200510595},
}

@incollection {Laptev2000,
    AUTHOR = {Laptev, Ari and Weidl, Timo},
     TITLE = {Recent results on {L}ieb-{T}hirring inequalities},
 BOOKTITLE = {Journ\'ees ``\'Equations aux {D}\'eriv\'ees {P}artielles''
              ({L}a {C}hapelle sur {E}rdre, 2000)},
     PAGES = {Exp. No. XX, 14},
 PUBLISHER = {Univ. Nantes, Nantes},
      YEAR = {2000},
      ISBN = {2-86939-157-9},
   MRCLASS = {81Q10 (35J10 35P15)},
  MRNUMBER = {1775696},
MRREVIEWER = {G\"unter\ Berger},
}

@article {Netrusov1996,
    AUTHOR = {Netrusov, Y. and Weidl, T.},
     TITLE = {On {L}ieb-{T}hirring inequalities for higher order operators
              with critical and subcritical powers},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {182},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {355--370},
      ISSN = {0010-3616,1432-0916},
   MRCLASS = {47F05 (35P15 47N50)},
  MRNUMBER = {1447297},
MRREVIEWER = {Yu.\ V.\ Egorov},
       URL = {http://projecteuclid.org/euclid.cmp/1104288152},
}

@book {Gazzola1991,
    AUTHOR = {Gazzola, Filippo and Grunau, Hans-Christoph and Sweers, Guido},
     TITLE = {Polyharmonic boundary value problems},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1991},
      NOTE = {Positivity preserving and nonlinear higher order elliptic
              equations in bounded domains},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {2010},
     PAGES = {xviii+423},
      ISBN = {978-3-642-12244-6},
   MRCLASS = {35-02 (31B30 35A08 35J40 35J61 46E35 58E12)},
  MRNUMBER = {2667016},
MRREVIEWER = {Rodney\ Josu\'e\ Biezuner},
       DOI = {10.1007/978-3-642-12245-3},
       URL = {https://doi.org/10.1007/978-3-642-12245-3},
}

@article{Grone1990,
  title={The Laplacian spectrum of a graph},
  author={Grone, Robert and Merris, Russell and Sunder, Viakalathur Shankar},
  journal={SIAM Journal on matrix analysis and applications},
  volume={11},
  number={2},
  pages={218--238},
  year={1990},
  publisher={SIAM}
}

@article{Guattery2000,
  title={Graph embeddings and laplacian eigenvalues},
  author={Guattery, Stephen and Miller, Gary L},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={21},
  number={3},
  pages={703--723},
  year={2000},
  publisher={SIAM}
}

@article{Hua2014,
  title={Harmonic functions of general graph Laplacians},
  author={Hua, Bobo and Keller, Matthias},
  journal={Calculus of Variations and Partial Differential Equations},
  volume={51},
  number={1},
  pages={343--362},
  year={2014},
  publisher={Springer}
}

@article{Bauer2022,
  title={Eigenvalue sum estimates for lattice subgraphs},
  author={Bauer, Frank and Lippner, Gabor},
  journal={Pure and Applied Mathematics Quarterly},
  volume={18},
  number={6},
  pages={2339--2353},
  year={2022},
  publisher={International Press of Boston}
}

@article{Hirschler2021,
  title={Laplace and bi-Laplace equations for directed networks and Markov chains},
  author={Hirschler, Thomas and Woess, Wolfgang},
  journal={Expositiones Mathematicae},
  volume={39},
  number={2},
  pages={271--301},
  year={2021},
  publisher={Elsevier}
}

@article{Duffin1958,
  title={Difference equations of polyharmonic type},
  author={Duffin, RJ and Shelly, EP},
  year={1958}
}

@article{Feng2012,
  title={Discrete bi-Laplacians and biharmonic B-splines},
  author={Feng, Powei and Warren, Joe},
  journal={ACM Transactions on Graphics (TOG)},
  volume={31},
  number={4},
  pages={1--11},
  year={2012},
  publisher={ACM New York, NY, USA}
}

@phdthesis{Schweiger2021,
  title={On the membrane model and the discrete Bilaplacian},
  author={Schweiger, Florian Martin},
  year={2021},
  school={Universit{\"a}ts-und Landesbibliothek Bonn}
}


@article{Khalkhuzhaev2019,
  title={Expansion of eigenvalues of rank-one perturbations of the discrete bilaplacian},
  author={Khalkhuzhaev, Ahmad and Kholmatov, Shokhrukh Yu and Pardabaev, Mardon},
  journal={arXiv preprint arXiv:1910.01369},
  year={2019}
}

@article{Wang2023,
  title={Eigenvalue estimates for the fractional Laplacian on lattice subgraphs},
  author={Wang, Jiaxuan},
  journal={arXiv preprint arXiv:2303.15766},
  year={2023}
}






